The planar directed k-Vertex-Disjoint Paths problem is fixed-parameter tractable

Given a graph G and k pairs of vertices (s_1,t_1), ..., (s_k,t_k), the k-Vertex-Disjoint Paths problem asks for pairwise vertex-disjoint paths P_1, ..., P_k such that P_i goes from s_i to t_i. Schrijver [SICOMP'94] proved that the k-Vertex-Disjoint Paths problem on planar directed graphs can be solved in time n^{O(k)}. We give an algorithm with running time 2^{2^{O(k^2)}} n^{O(1)} for the problem, that is, we show the fixed-parameter tractability of the problem.

==> old-top-r-decomposition.tex <==
\newcommand{\anycomp}{\ensuremath{\mathbf{C}}}
\newcommand{\disccomp}{\ensuremath{\mathbf{C}^{\textrm{disc}}}}
\newcommand{\ringcomp}{\ensuremath{\mathbf{C}^{\textrm{ring}}}}
\newcommand{\decomp}{\ensuremath{\mathcal{D}}}

\section{Decomposition}

We start with defining the notion of components in our decomposition.
We decide to state them as topological objects on the plane (parts of a graph surrounded by some curves)
to make later homotopy-based arguments easier.

\begin{defin}[border noose]
  Let $G$ be a graph embedded in the plane. A noose $N$ is called a {\em{border noose}} if it does not intersect itself and does not contain any vertex of $G$.
\end{defin}

\begin{defin}[disc component]
Let $G$ be a graph embedded in the plane and let $N$ be a border noose. Then:
\begin{itemize}
\item the subgraph of $G$ that consists of vertices and edges completely contained in the
area inside $N$ is called a {\em{disc component with border $N$}};
\item the area enclosed by $N$ is called the {\em{area of the component}};
\item the {\em{alternation}} of the disc component is the alternation of its border.
\end{itemize}
\end{defin}

\begin{defin}[ring component]
Let $G$ be a graph embedded in the plane and let $N_{IN}$ and $N_{OUT}$ be two border disjoint border nooses
such that $N_{IN}$ lies inside the area enclosed by $N_{OUT}$.
Then:
\begin{itemize}
\item the subgraph of $G$ that consists of vertices and edges completely contained in the area between $N_{IN}$ and $N_{OUT}$
is called a {\em{ring component with inner border $N_{IN}$ and outer border $N_{OUT}$}};
\item the area enclosed between $N_{IN}$ and $N_{OUT}$ is called the {\em{area of the component}};
\item the {\em{alternation}} of the disc component is the maximum of the alternations of its borders.
\end{itemize}
\end{defin}

Please note that a (disc or ring) component of a graph may contain many connected components.
  Moreover, they may exist an edge of $G$ that has both endpoints in a single component of $G$, but does not belong to this component.
  This happens if this edge crosses the border of the component.

\begin{defin}[decomposition]
  Let $G$ be a graph embedded in the plane having a set $T\subseteq
  V(G)$ of terminals. 
  Then a set $\decomp$ of (disc and ring) components of $G$ is a {\em{decomposition}} of $G$ iff
  \begin{itemize}
   \item every vertex of $G$ is in exactly one component of $\decomp$;
   \item the areas of components are pairwise disjoint;
   \item for each terminal $t \in T$ there exists a disc component $\disccomp_t \in \decomp$ that consists of the vertex $t$ only.
  \end{itemize}

   The {\em{(disc, ring) alternation}} of the decomposition $\decomp$ is the maximum alternation of a (disc, ring) component in $\decomp$.
\end{defin}
We will control two natural measures of a quality of a decomposition: its alternation and the number of its components.
Moreover, we will require that ring components are embedded into a decomposition in a special way.

\begin{defin}[isolating component]
Consider a decomposition $\decomp$ of an embedded graph $G$ with terminals $T$. We say that a disc component $\disccomp \in \decomp$
is a {\em{$d$-isolating}} component if the subgraph of $G$ induced by the vertices of $\disccomp$ (i.e., the subgraph $\disccomp$ together
    with all the edges of $G$ that have both endpoints in $\disccomp$ but cross the edge of $\disccomp$)
contains a sequence of $d$ alternating cycles and each edge of $G$ that has exactly one endpoint in $G$ either lies inside the innermost of these cycles (an {\em{inner edge}})
or lies outside the outermost of these cycles (an {\em{outer edge}}).
\end{defin}

\begin{defin}[ring isolation]\label{def:isolation}
Consider a decomposition $\decomp$ of an embedded graph $G$ with terminals $T$. We say that the decomposition has {\em ring isolation $d$}
if for every ring component $\ringcomp \in \decomp$ with inner border $N_{IN}$ and outer border $N_{OUT}$ there exist two $d$-isolating
  disc components $\disccomp_{IN}$ and $\disccomp_{OUT}$ such that:
 \begin{itemize}
   \item the component $\disccomp_{IN}$ is contained inside $N_{IN}$ and
     each edge of $G$ that has exactly one endpoint in $\disccomp_{IN}$ is an outer edge if and only if it has the second endpoint in $\ringcomp$;
   \item the component $\disccomp_{OUT}$ is contained outside $N_{OUT}$ and
     each edge of $G$ that has exactly one endpoint in $\disccomp_{OUT}$ is an inner edge if and only if it has the second endpoint in $\ringcomp$;
   \item each edge with exactly one endpoint in $\ringcomp$ either crosses $N_{IN}$ and has the second endpoint in $\disccomp_{IN}$
     or crosses $N_{OUT}$ and has the second endpoint in $\disccomp_{OUT}$.
 \end{itemize}
\end{defin}

We are now ready to state our decomposition theorem.

\begin{theorem}[Main Decomposition Theorem]\label{th:finddecomp}
Let $G$ be an embedded graph with $k$ terminals, each of them having degree 1.
Let $d$ and $r$ be integers and let $q=q(r)$ and $x=x(r)$ be bounds given by
Lemma \ref{lem:largering}.
Then in $O^*(2^{O((x+q+d)k^2)})$ time we can either find a set
of $r$ concentric cycles with no terminal inside the outermost
cycle, or compute a set of at most $2^{O((x+q+d)k^2)}$ pairs $(E_i, \decomp_i)$ where:
\begin{enumerate}
\item $E_i \subseteq E(G)$;
\item $\decomp_i$ is a decomposition of the graph $G \setminus E_i$ with $O(k^2)$ components, ring isolation $d$, disc alternation $O(kx+(q+d)k^2)$ and ring alternation $x$;
\item if $G$ is a yes instance, then there exists a solution and an index $i$ such that the solution is disjoint with $E_i$.
\end{enumerate}
\end{theorem}

\begin{proof}
We decompose the graph in a recursive manner. At each step
we are given a border noose and we are to decompose the disc component inside it.
We start with a border noose that surrounds the entire graph $G$; note that this
noose has alternation $-1$.

Denote the current component to decompose as $\disccomp$ with border $N$.
If $\disccomp$ does not contain any terminal, we return it as a single disc component with border $N$.
If there is a terminal on the outer face of $\disccomp$, we create a new disc component that contains it
and modify $N$ to remove the terminal and its incident edge from $\disccomp$. 
This step produces at most $|T|=k$ disc components in the entire decomposition algorithm.

Thus, from this point we may assume that $\disccomp$ contains $\kappa > 0$ terminals, but none of these terminals lie in the outer face of $\disccomp$.
Let us pick one terminal $t \in T \cap V(\disccomp)$ and let $F_t$ be the face that contains $t$. Let $\gamma_t$ be an arbitrary circle with centre $t$ and with sufficiently
small radius such that $\gamma_t$ is contained in $F_t$ and is a border noose surrounding
$t$. Invoke Lemma \ref{lem:dualcycles} on curves $\gamma_t$ and $N$ 
and find largest even $a$ for which we obtain a sequence $C_1,C_2, \ldots, C_a$
of alternating concentric cycles in $\disccomp$. Moreover, invoke
Lemma \ref{lem:dualcycles} for $a+2$ and obtain a simple curve $M$ connecting $\gamma_t$ and $N$ with at most $a+2$
alternations.

Assume $C_1$ is the innermost and $C_a$ is the outermost
of the constructed cycles. For $s=1,2,\ldots,\kappa$
let $i(s)$ be the largest integer $0 \leq i(s) \leq a$ such that
there are at most $s$ terminals contained in the area
enclosed by the cycle $C_{i(s)}$ (note that no terminal lies on any of the cycles $C_1,C_2, \ldots, C_a$, as terminals are of degree one in $G$). Note that $i(\kappa) = a$; we
denote $i(0) = 0$.

Let $S^{\textrm{big}} \subseteq \{1,2,\ldots,\kappa\}$ be the set of those
integers such that $s \in S^{\textrm{big}}$ whenever $i(s) - i(s-1) > 2d+4q$,
where $q=q(r)$ is the bound given by Lemma \ref{lem:largering}.
For each $s \in S^{\textrm{big}}$, apply Lemma \ref{lem:largering} to the following
four sets of $q+1$ concentric cycles:
\begin{itemize}
\item $C_{i(s-1)+1}, C_{i(s-1)+2}, \ldots, C_{i(s-1)+q+1}$;
\item $C_{i(s-1)+q+d}, C_{i(s-1)+q+d+2}, \ldots, C_{i(s-1)+2q+d}$;
\item $C_{i(s)-2q-d + 1}, C_{i(s)-2q-d+2}, \ldots, C_{i(s)-q-d+1}$;
\item $C_{i(s)-q}, C_{i(s)-q+2}, \ldots, C_{i(s)}$.
\end{itemize}
If any of the applications of Lemma \ref{lem:largering} returns
  a sequence of $r$ concentric cycles, we return it as an outcome of the algorithm.
Otherwise, we obtain four circular cuts $N_s^1, N_s^2, N_s^3$ and $N_s^4$.
Note that the $d$ cycles $C_{i(s-1)+q+1}, C_{i(s-1)+q+2}, \ldots, C_{i(s-1)+q+d}$
are contained between $N_s^1$ and $N_s^2$, whereas 
the $d$ cycles $C_{i(s)-q-d+1}, C_{i(s)-q-d+2}, \ldots, C_{i(s)-q}$ are contained
between $N_s^3$ and $N_s^4$.

As the simple curve $M$ connects $\gamma_t$ with $N$, it crosses all cycles $C_i$
as well as all circular cuts $N_s^\alpha$ for $s \in S^{\textrm{big}}$,
$1 \leq \alpha \leq 4$. By slightly perturbing $M$, we may assume that
$M$ crosses these circular cuts either in a vertex of $G$ or inside a face of $G$,
  never on an edge of $G$.
For each $s \in S^{\textrm{big}}$, remove from
$M$ the subcurve between the intersection with $N_s^2$ that is closest to $\gamma_t$
on $M$ and the intersection with $N_s^3$ that is closest to $N$ on $M$;
if the intersection happens in the vertex of $G$, we remove a slightly shorter
part of $M$, so that the remaining curve still traverses the intersection vertex
and ends in a face of $G$.
Denote by $\mathcal{M}$ the set of remaining subcurves of $M$ (note that
the are at most $|S^{\textrm{big}}|+1 \leq \kappa+1$ of them).

We now note that all curves in $\mathcal{M}$ intersect at most $(4q+2d)\kappa$ alternating
cycles from the sequence $C_1,C_2,\ldots, C_a$, as they intersect at most
$4q+2d$ cycles between $C_{i(s-1)+1}$ and $C_{i(s)}$ for each $1 \leq s \leq \kappa$.
Recall that the alternation of $M$ is at most $a+2$, while $M$ intersects
all cycles $C_1,C_2,\ldots, C_a$. Therefore the sum of alternations of all curves
in $\mathcal{M}$ is at most $(4q+2d)\kappa+2$.\footnote{MP: Do we want to prove it more formally? The claim is obvious up to lower order terms. But, as $|\mathcal{M}|$ is bounded,
  we may even afford to lose something on alternation on each curve.}

We are now going to cut the graph along the circular cuts $N_s^\alpha$ for $s \in S^\textrm{big}$, $1 \leq \alpha \leq 4$, as well as along the curves of $\mathcal{M}$.
However, both circular cuts and the curves in $\mathcal{M}$ may traverse a vertex, whereas
the borders of the components are allowed to cut edges only.
To cope with this, we introduce the following bounded search tree strategy.

Recall that any curve of $\mathcal{M}$ as well as any cut $N_s^\alpha$ is
a simple curve. Let $N_0$ be any of these curves, and let $v$ be a vertex on $N_0$.
By the defiintion of a simple curve, the set $S_v \in \snoose(N_0)$ that corresponds
to $v$ equals $\{+1,-1\}$ or $\emptyset$.

For a given curve $N_0$, we first resolve all vertices with $S_v = \{+1,-1\}$.
For each such vertex, we branch into four cases. We choose one side of
the curve $N_0$ (left or right) around the vertex $v$ and one type of arcs incident to $v$
(incoming or outgoing arcs). In each branch, we delete from the graph the arcs
of the chosen type from the chosen side of the curve (and put them into the set
$E_i$ for the current branch) and perturb $N_0$ slightly to omit the vertex $v$ from the
chosen side. In this way, we do not increase $\alt(N_0)$, as
in $\snoose(N_0)$ we exchange the $S_v = \{+1,-1\}$ 
for a sequence (of arbitrary length) of equal one-element sets, corresponding
to the remaining arcs from the chosen side of $N_0$. 
Moreover, for any solution to the \textsc{Disjoint Paths} problem,
there exists a choice where we do not delete any arcs of the solution,
as the vertex $v$ may lie only on one path of the solution, and these path
cannot enter and leave the vertex $v$ from both sides of $N_0$.

Note that the number of these vertices is at most $\alt(N_0)+1$, thus we create 
at most $4^{\alt(N_0)+1}$ branches.

Once we have resolved all vertices with $S_v = \{+1,-1\}$, we move to the second
case. For a vertex $v$ we may have $S_v = \emptyset$ in two situations.
First, $N_0$ may visit vertex $v$, but 
leaves all incident edges on one of its sides. In this situation, we may simply move $N_0$
a bit, in order not to visit $v$.

Second, $v$ may be a source or a sink. We consider here two options: either we modify
the curve $N_0$ to omit the vertex $v$ from the left or from the right.
Let us investigate how such a change will influence $\snoose(N_0)$ and $\alt(N_0)$.
We replace $S_v = \emptyset$ with a sequence (of arbitrary length) of equal one-element
sets corresponding to the traversed arcs of $G$; such a situation may increase $\alt(N_0)$
by one. However, we have a choice of whether we insert a sequence of sets $\{+1\}$
or $\{-1\}$: if we omit the vertex $v$ from the left, we cross the arcs incident
to it in a different orientation than if we omit the vertex $v$ from the right.

If in $\snoose(N_0)$ there exists a vertex $v$ with $S_v = \emptyset$, but one neighbouring
set $S$ with $|S|=1$, we may modify $N_0$ around $v$ so that we replace $S_v$
with a sequence of sets equal to $S$; this operation does not increase $\alt(N_0)$.
As we have removed all two-element sets from $\snoose(N_0)$, we may not perform
the above operation only if $\snoose(N_0)$ consists only of empty sets. In this case,
we modify $N_0$ around each vertex, so that $\snoose(N_0)$ is a sequence of sets $\{+1\}$;
note that the alternation of $N_0$ changes from $-1$ to $0$ in this case.

Let us now summarize. Recall that:
\begin{itemize}
\item $|\mathcal{M}| \leq \kappa+1$;
\item there are at most $4\kappa$ curves
  $N_s^\alpha$, $s \in S^{\textrm{big}}$, $1 \leq \alpha \leq 4$;
\item the sum of alternations of all curves of $\mathcal{M}$ is at most $(4q+2d)\kappa$;
\item each curve $N_s^\alpha$ has alternation at most $x = x(r)$ (given
  by Lemma \ref{lem:largering}).
\end{itemize}
Therefore the aforementioned procedure generates at most
$4^{(4x + 4q + 2d + 5)\kappa+1}$ subcases, and increases alternation
of each curve by at most one.

We now partition the graph into the following components.
\begin{itemize}
\item We create a disc component with border $\gamma_t$ containing the terminal $t$
only.
\item For each $s \in S^\textrm{big}$, we create:
  \begin{itemize}
  \item a ring component $\ringcomp_s$ with inner border $N_s^2$ and outer
  border $N_s^3$;
  \item a disc component $\disccomp_{s,IN}$
  with border being a concatenation of the following four
  curves: a minimal segment of a curve of $\mathcal{M}$ connecting $N_s^1$ with $N_s^2$,
  the curve $N_s^2$, the same minimal segment of a curve of $\mathcal{M}$,
  but now traversed backwards, and the curve $N_s^1$; we perturb slightly all the parts of the border
  in order to make them disjoint with the original curves;
  note that this disc component contains all the vertices and edges of $G$ that lie between
  $N_s^1$ and $N_s^2$, except for the edges that intersect $N_s^1$, $N_s^2$ or the chosen curve that connects $N_s^1$ and $N_s^2$;
  \item a second disc component $\disccomp_{s,OUT}$,
  created in the same manner as the aforementioned one,
  but between curves $N_s^3$ and $N_s^4$.
  \end{itemize}
  We note that the alternating cycles $C_{i(s-1)+q+1}, C_{i(s-1)+q+2},\ldots,C_{i(s-1)+q+d}$
  are contained in the subgraph of $G$ induced by the vertices of $\disccomp_{s,IN}$,
  fulfilling all the requirements to make $\disccomp_{s,IN}$ a $d$-isolating component.
  Similarly the cycles $C_{i(s)-q-d+1},C_{i(s)-q-d+2},\ldots, C_{i(s)-q}$ make
  $\disccomp_{s,OUT}$ a $d$-isolating component. Therefore $\ringcomp_s$ has
  proper isolation.
\item For each $s \in S^\textrm{big} \cup \{a+1\}$, we recursively invoke the
  decomposition algorithm to the subgraph enclosed by the following noose.
  We denote $N_0^4 = \gamma_t$ and $N_{a+1}^1 = N$. We concatenate
  a minimal segment of a curve of $\mathcal{M}$ connecting $N_{s-1}^4$ and
  $N_s^1$, the curve $N_s^1$, again the same minimal segment but traversed backwards,
  and the curve $N_{s-1}^4$. Once again, we perturb slightly the parts of the noose
  to make them disjoint with the borders of the neighbouring components.
\end{itemize}
Note that, after this step, the total number of terminals in the recursive
calls is at most $\kappa-1$, as the terminal $t$ is put in its own disc component
and each other terminal is put into exactly one new recursive call.
Therefore, the depth of the recursion is at most $k$.
Moreover, as the step creates at most $\kappa$ ring components
and $2\kappa$ disc components that are not components with a terminal,
we obtain at most $O(k^2)$ components in total
and at most $2^{O((x+q+d)k^2)}$ subcases.

Let us now bound the alternations of the constructed components.
Each constructed ring component $\ringcomp_s$
has two borders $N_s^2$ and $N_s^3$ of alternation at most $x$,
 thus its alternation is at most $x$.
The border of each isolating component $\disccomp_{s,IN}$ and $\disccomp_{s,OUT}$
consists of two circular cuts of alternation $x$ each and two subcurves of a
curve of $\mathcal{M}$. Recall that the sum of alternations of all curves
in $\mathcal{M}$ is at most $(2d+4q)\kappa$, thus each isolating disc component
has alternation $O(x+(d+q)k)$.
Moreover, $\gamma_t$ has alternation $0$.

In each recursive call, we invoke the algorithm on a component with border
consisting of two copies of a subcurve of a curve from $\mathcal{M}$
and two nooses being either circular cuts $N_s^\alpha$, the curve $\gamma_t$ or $N$.
A operation of cutting away a disc component with a terminal may increase
the alternation of $N$ by at most one per terminal, thus $k$ in total.
We infer that at recursion depth $i$, the noose $N$ has alternation
bounded by $O(i(x+(d+q)k))$. Therefore,
  if the recursion stops returning a single disc component
(i.e., if there is no terminal inside the area enclosed by $N$),
  the returned disc component has alternation $O(xk + (d+q)k^2)$.

This concludes the proof of the decomposition theorem.
\end{proof}



